Joint Beamforming and Matching for Ultra-Dense Massive Antenna Arrays

Massive multiple-input multiple-output (MIMO) offers substantial spectral-efficiency gains, but scaling to very large antenna arrays with conventional all-digital and hybrid beamforming architectures quickly results in excessively high costs and power consumption. Low-cost, switch-based architectures have recently emerged as a potential alternative. However, prior studies rely on simplified models that ignore (among others) antenna coupling, radiation patterns, and matching losses, resulting in inaccurate performance predictions. In this paper, we use a physically consistent electromagnetic modeling framework to analyze an ultra-dense patch-antenna array architecture that performs joint beamforming and matching using networks of inexpensive RF switches. Our results demonstrate that simple, switch-based beamforming architectures can approach the antenna-gain of all-digital solutions at significantly lower cost and complexity.

==> sty/eth-colours.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% ETH Zürich's Corporate Design Colours
%%
%% Alexander Stutz (alstutz@iis.ee.ethz.ch)
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% corporate design colours
\definecolor{eth_blue}{RGB}{33, 92, 175}
\definecolor{eth_blue_10}{RGB}{233, 239, 247}
\definecolor{eth_blue_20}{RGB}{211, 222, 239}
\definecolor{eth_blue_60}{RGB}{122, 157, 207}
\definecolor{eth_blue_80}{RGB}{77, 125, 191}
\definecolor{eth_blue_120}{RGB}{8, 64, 126}

\definecolor{eth_petrol_120}{RGB}{0, 89, 109}
\definecolor{eth_petrol}{RGB}{0, 120, 148}
\definecolor{eth_petrol_10}{RGB}{231, 244, 247}
\definecolor{eth_petrol_20}{RGB}{204, 228, 234}

\definecolor{eth_green_120}{RGB}{60, 81, 30}
\definecolor{eth_green}{RGB}{98, 115, 19}
\definecolor{eth_green_10}{RGB}{239, 241, 231}
\definecolor{eth_green_20}{RGB}{224, 227, 208}
\definecolor{eth_green_60}{RGB}{161, 171, 113}
\definecolor{eth_green_80}{RGB}{129, 143, 66}
\definecolor{eth_green_120}{RGB}{54, 82, 19}

\definecolor{eth_bronze_120}{RGB}{107, 80, 31}
\definecolor{eth_bronze}{RGB}{142, 103, 19}
\definecolor{eth_bronze_10}{RGB}{244, 240, 231}

\definecolor{eth_red_120}{RGB}{150, 39, 45}
\definecolor{eth_red}{RGB}{183, 53, 45}
\definecolor{eth_red_80}{RGB}{197, 93, 87}
\definecolor{eth_red_10}{RGB}{248, 235, 234}
\definecolor{eth_red_20}{RGB}{241,215,213}

\definecolor{eth_purple_120}{RGB}{140, 10, 89}
\definecolor{eth_purple}{RGB}{167, 17, 122}
\definecolor{eth_purple_10}{RGB}{248, 232, 243}
\definecolor{eth_purple_20}{RGB}{239, 208, 227}

\definecolor{eth_grey_120}{RGB}{87, 87, 87}
\definecolor{eth_grey}{RGB}{111, 111, 111}
\definecolor{eth_grey_10}{RGB}{241, 241, 241}


% black and shades of grey
% (for non-white background check required opacity online)
\definecolor{eth_black}{RGB}{0, 0, 0}
\definecolor{eth_black_light}{RGB}{34, 34, 34}
\definecolor{eth_black_60}{RGB}{102, 102, 102}
\definecolor{eth_black_light_48}{RGB}{149,149,149}
\definecolor{eth_black_light_20}{RGB}{211, 211, 211}
\definecolor{eth_grey_10}{RGB}{241, 241, 241}
\definecolor{eth_grey_05}{RGB}{246, 246, 246}






==> sty/macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% Macros for the Paper 
%%
%% "Efficient and Physically-Consistent Modeling
%%  of Reconfigurable Electromagnetic Structures"
%%
%% Alexander Stutz, Georg Schwan, and Christoph Studer
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Color Palette:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{sty/eth-colours}

% corporate design colors
\colorlet{blue}{eth_blue}
\colorlet{blue_10}{eth_blue_10}
\colorlet{blue_20}{eth_blue_20}
\colorlet{blue_60}{eth_blue_60}
\colorlet{blue_80}{eth_blue_80}
\colorlet{blue_120}{eth_blue_120}

\colorlet{petrol_120}{eth_petrol_120}
\colorlet{petrol}{eth_petrol}
\colorlet{petrol_10}{eth_petrol_10}
\colorlet{petrol_20}{eth_petrol_20}

\colorlet{green_120}{eth_green_120}
\colorlet{green}{eth_green}
\colorlet{green_10}{eth_green_10}
\colorlet{green_60}{eth_green_60}
\colorlet{green_80}{eth_green_80}
\colorlet{green_120}{eth_green_120}

\colorlet{bronze_120}{eth_bronze_120}
\colorlet{bronze}{eth_bronze}
\colorlet{bronze_10}{eth_bronze_10}

\colorlet{red_120}{eth_red_120}
\colorlet{red}{eth_red}
\colorlet{red_80}{eth_red_80}
\colorlet{red_10}{eth_red_10}

\colorlet{purple_120}{eth_purple_120}
\colorlet{purple}{eth_purple}
\colorlet{purple_10}{eth_purple_10}
\colorlet{purple_20}{eth_purple_20}

\colorlet{black}{eth_black}
\colorlet{black_light}{eth_black_light}
\colorlet{black_60}{eth_black_60}
\colorlet{black_light_48}{eth_black_light_48}
\colorlet{black_light_20}{eth_black_light_20}
\colorlet{grey_120}{eth_grey_120}
\colorlet{grey}{eth_grey}
\colorlet{grey_10}{eth_grey_10}
\colorlet{grey_05}{eth_grey_05}

\definecolor{pink}{RGB}{214,82,130}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Tikz Macros:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfdeclarepatternformonly{south east lines my}{\pgfqpoint{-0pt}{-0pt}}{\pgfqpoint{5pt}{5pt}}{\pgfqpoint{5pt}{5pt}}{
    \pgfsetlinewidth{0.5pt}
    \pgfpathmoveto{\pgfqpoint{0pt}{5pt}}
    \pgfpathlineto{\pgfqpoint{5pt}{0pt}}
    \pgfpathmoveto{\pgfqpoint{.2pt}{-.2pt}}
    \pgfpathlineto{\pgfqpoint{-.2pt}{.2pt}}
    \pgfpathmoveto{\pgfqpoint{5.2pt}{4.8pt}}
    \pgfpathlineto{\pgfqpoint{4.8pt}{5.2pt}}
    \pgfusepath{stroke}}
    
\pgfdeclarepatternformonly{horizontal lines my}{\pgfqpoint{-0pt}{-0pt}}{\pgfqpoint{3.54pt}{3.54pt}}{\pgfqpoint{3.54pt}{3.54pt}}{
    \pgfsetlinewidth{0.5pt}
    \pgfpathmoveto{\pgfqpoint{0pt}{2pt}}
    \pgfpathlineto{\pgfqpoint{3.54pt}{2pt}}
    \pgfusepath{stroke}}

\pgfdeclarepatternformonly{diagonal behind text}{\pgfqpoint{-0pt}{-0pt}}{\pgfqpoint{15pt}{15pt}}{\pgfqpoint{15pt}{15pt}}{
    \pgfsetlinewidth{0.7pt}
    \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
    \pgfpathlineto{\pgfqpoint{15pt}{15pt}}
    \pgfpathmoveto{\pgfqpoint{14.8pt}{-.2pt}}
    \pgfpathlineto{\pgfqpoint{15.2pt}{.2pt}}
    \pgfpathmoveto{\pgfqpoint{-.2pt}{14.8pt}}
    \pgfpathlineto{\pgfqpoint{.2pt}{15.2pt}}
    \pgfusepath{stroke}}

\pgfdeclarepatternformonly{diagonal pattern node}{\pgfqpoint{-0pt}{-0pt}}{\pgfqpoint{3pt}{3pt}}{\pgfqpoint{3pt}{3pt}}{
    \pgfsetlinewidth{0.7pt}
    \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
    \pgfpathlineto{\pgfqpoint{3pt}{3pt}}
    \pgfpathmoveto{\pgfqpoint{2.8pt}{-.2pt}}
    \pgfpathlineto{\pgfqpoint{3.2pt}{.2pt}}
    \pgfpathmoveto{\pgfqpoint{-.2pt}{2.8pt}}
    \pgfpathlineto{\pgfqpoint{.2pt}{3.2pt}}
    \pgfusepath{stroke}}

\def\centerOfC at (#1,#2){
    \draw  [shift={(#1,#2)}, rotate=-45,line width=0pt, fill=white, color=white, anchor=center] (-.27,-.27) rectangle (.27,.27);
    \draw  [shift={(#1,#2)}, rotate=-45,line width=0pt, fill=white, color=white, anchor=center] (-.3,-.15) rectangle (.3,.15);

    
    \draw  [shift={(#1,#2)},line width=0.3pt, fill=white] (0,0) ellipse (0.16 and 0.16);
    \draw [shift={(#1,#2)},line width=0.3pt, color=black] (-0.2,0) -- (0.2,0);
    \draw [shift={(#1,#2)},line width=0.3pt, color=black] (0,-0.2) -- (0,0.2);
    \draw [shift={(#1,#2)},line width=0.3pt, color=black, fill=black]  (0,0) -- (0:0.16) arc (0:90:.16) -- cycle;
    \draw [shift={(#1,#2)},line width=0.3pt, color=black, fill=black]  (0,0) -- (180:0.16) arc (180:90+180:.16) -- cycle;
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Operators:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareMathOperator{\diag}{diag}			        % diag matrix
\DeclareMathOperator{\Ex}{\mathbb{E}}		        % expectation operator
\newcommand{\T}[0]{\mathsf{T}}                      % transpose
\newcommand{\He}[0]{\mathsf{H}}                     % hermitian
\DeclareMathOperator*{\argmax}{arg\,max}            % argmax
\DeclareMathOperator*{\maximize}{maximize}          % maximize               

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Font Macros:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\up}[1]{{\textnormal{#1}}}              % subscripts
\newcommand{\upc}[1]{{\textnormal{\textbf{#1}}}}    % subscripts in caption

\newcommand{\mat}[1]{{\bm{\mathbf{#1}}}}            % matrices
\newcommand{\vect}[1]{{\bm{\mathbf{#1}}}}           % vectors
\newcommand{\oper}[1]{\mathbb{#1}}                  % operator

\newcommand{\phs}[1]{{\color{pink}\mathsf{#1}}}  % phasor scalar
\newcommand{\phv}[1]{{\color{pink}\bm{\mathsf{#1}}}} % phasor vector





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Fancy Ref Stuff
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand*{\fancyrefapplabelprefix}{app}		% Appendix
\newcommand*{\fancyrefthmlabelprefix}{thm}		% Theorem
\newcommand*{\fancyrefdefilabelprefix}{defi}    % Definition
\newcommand*{\fancyrefproplabelprefix}{prop}	% Proposition
\newcommand*{\fancyrefalglabelprefix}{alg}		% Algorithm
\newcommand*{\fancyrefasmlabelprefix}{asm}		% Assumption
\newcommand*{\fancyrefremlabelprefix}{rem}		% Remark


% label names
\frefformat{vario}{\fancyrefseclabelprefix}{Sec.~#1}
\frefformat{vario}{\fancyrefthmlabelprefix}{Thm.~#1}
\frefformat{vario}{\fancyrefdefilabelprefix}{Def.~#1}
\frefformat{vario}{\fancyreffiglabelprefix}{Fig.~#1}
\frefformat{vario}{\fancyrefapplabelprefix}{App.~#1}
\frefformat{vario}{\fancyrefeqlabelprefix}{(#1)}
\frefformat{vario}{\fancyrefproplabelprefix}{Prop.~#1}
\frefformat{vario}{\fancyrefalglabelprefix}{Alg.~#1}
\frefformat{vario}{\fancyrefasmlabelprefix}{Assu.~#1}
\frefformat{vario}{\fancyrefremlabelprefix}{Rem.~#1}
